Future Advances in Photon-Based Neutrino Detectors: A SNOWMASS White Paper

We discuss here new, enabling technologies for future photon-based neutrino detectors. These technologies touch nearly every aspect of such detectors: new scintillating materials, new methods of loading isotopes, new photon sensors and collectors, new approaches to simulation and analysis, and new front-end electronics and DAQ ideas. Of particular interest are technologies that enable broad physics programs in hybrid Cherenkov/scintillation detectors, such as slow fluors, water-based liquid scintillator, and spectral sorting of photons. Several new large-scale detector ideas are also discussed, including hybrid detectors like Theia, ArTEMIS, and generic slow-fluor detectors, as well as the very different SLIPs and LiquidO approaches to instrumenting photon-based detectors. A program of demonstrators for future detectors, including ANNIE, Eos, and NuDOT are also discussed.

==> photons_AuthorList_orig.tex <==
\newcommand{\Editor}{Editor.}
\newcommand{\Contributor}{Primary Contributor.}
%% Do not edit above this line!
%%============================================
%%=========== Instructions ===================
% 1) Add a “newcommand" for any new affiliation in the first block of commands below, please make sure it is added in alphabetical order of institution's name. Can be skipped only if the affiliation already exists.

% 2) Add an \affiliation directive in the same alphabetical order as in 1) to the second block of commands below. Can be skipped only if the affiliation already exists.

% 3) Add author(s) with affiliation(s) in alphabetical order of the author's last name to the 3rd block of commands. 
% 4) Press the “Recompile” button and make sure you see an author list and the authors and affiliations you entered. If not, look through your changes, fix any errors, and recompile again.
%%=========== End of Instructionsش =============

%Authors go here with affiliation indexed by [X]
% 1st Block of Commands
%Please enter a newcommand per affiliation, please make sure they are entered in alphabetical order of institution name. 
\newcommand{\UA}{University at Albany, State University of New New York (SUNY), Albany, NY USA}
\newcommand{\ANL}{Argonne National Laboratory, IL, USA}
\newcommand{\APC}{Université de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}
\newcommand{\Atlantico}{Universidad del Atl\'antico, Puerto Colombia, Atl\'antico, Colombia}
\newcommand{\UBERN}{Universt\"at Bern, Bern, Switzerland}
\newcommand{\BEU}{Beykent University, Istanbul, Turkey}
\newcommand{\BU}{Boston University, Boston, MA, USA}
\newcommand{\BNL}{Brookhaven National Laboratory, NY, USA}
\newcommand{\BHU}{Banaras Hindu University, Varanasi, INDIA}
\newcommand{\UoBham}{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\newcommand{\UB}{University of Bristol, Bristol BS8 1TL, United Kingdom}
\newcommand{\UoB}{University of Bucharest, Bucharest, Romania}
\newcommand{\Caltech}{California Institute of Technology, Pasadena, CA, USA}
\newcommand{\UCB}{University of California, Berkeley, Berkeley, CA USA}
\newcommand{\UCD}{University of California, Davis, Davis, CA USA}
\newcommand{\UNC}{University of North Carolina, Chapel Hill, NC USA}
\newcommand{\UCI}{University of California, Irvine, CA, USA}
\newcommand{\JGU}{Johannes Gutenberg University, Mainz, Germany}
\newcommand{\UCSB}{University of California, Santa Barbara, Santa Barbara, CA USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\Catania}{University and INFN Sezione di Catania, Catania, Italy}
\newcommand{\CERN}{CERN, 1 Esplanade des Particules, Geneva, Switzerland}
\newcommand{\CIEMAT}{CIEMAT, Centro de Investigaciones Energéticas, Medioambientales y Tecnólogicas, Madrid, Spain}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH, USA}
\newcommand{\CUSB}{Central University of South Bihar, Gaya, INDIA}
\newcommand{\Cinvestav}{Centro de Investigación y de Estudios Avanzados del Instituto Politécnico Nacional (Cinvestav), Mexico City, Mexico}
\newcommand{\Columbia}{Columbia University, New York, NY, USA}
\newcommand{\CSU}{Colorado State University, Fort Collins, CO, USA}
\newcommand{\Duke}{Duke University, Durham, NC, USA}
\newcommand{\Drexel}{Drexel University, Philadelphia, PA, USA}
\newcommand{\EDI}{University of Edinburgh, Edinburgh EH8 9YL, United Kingdom}
\newcommand{\EIA}{Universidad EIA, Envigado, Antioquia, Colombia}
\newcommand{\FCUL}{Faculdade de Ci\^{e}ncias da Universidade de Lisboa, Lisboa, Portugal}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL, USA}
\newcommand{\UF}{University of Florida, Gainesville, FL 32611, USA}
\newcommand{\UGR}{University of Granada \& CAFPE, Granada, Spain}
\newcommand{\Harvard}{Harvard University, Cambridge, MA, USA}
\newcommand{\Hawaii}{University of Hawaii, Honolulu, HI, USA}
\newcommand{\Houston}{University of Houston, Houston, TX, USA}
\newcommand{\ISU}{Idaho State University, Pocatello, ID, USA} 
\newcommand{\IU}{Indiana University, Bloomington, IN, USA} 
\newcommand{\IFIC}{Instituto de F\'isica Corpuscular (IFIC), CSIC \& Universitat de Val\`encia, Paterna, Spain}
\newcommand{\IIT}{Illinois Institute of Technology, Chicago, IL, USA}
\newcommand{\IITH}{Indian Institute of Technology Hyderabad, Kandi, Sangareddy, India}
\newcommand{\CzechAcademyofSciences}{Institute of Physics, Czech Academy of Sciences, 182 00 Prague 8, Czech Republic}
\newcommand{\INFNMi}{Istituto Nazionale di Fisica Nucleare, Sezione di Milano, Milano, Italy}
\newcommand{\INFNMiB}{Istituto Nazionale di Fisica Nucleare, Sezione di Milano Bicocca, Milano, Italy}
\newcommand{\INFNGE}{Istituto Nazionale di Fisica Nucleare, Sezione di Genova, Genova, Italy}
\newcommand{\INFNNA}{Universit\`a degli Studi di Napoli ``Federico II'' \& Istituto Nazionale di Fisica Nucleare, Sezione di Napoli, Napoli, Italy}
\newcommand{\Insubria}{Universit{\`a} degli Studi dell'Insubria, Dipartimento di Scienza e Alta Tecnologia, Como, Italy}
\newcommand{\UOH}{University of Hyderabad, Hyderabad - 500046, India}
\newcommand{\Iowa}{University of Iowa, Iowa City, IA, USA}
\newcommand{\ISP}{Instituto Superior Técnico, Lisbon, Portugal}
\newcommand{\IowaU}{Iowa State University, Ames, IA, USA}
\newcommand{\Irfu}{IRFU, CEA Saclay, Gif-sur-Yvette, France}
\newcommand{\Iwate}{Iwate University, Morioka, Iwate, Japan}
\newcommand{\JBNU}{Jeonbuk National University, Jeonju, Jeonbuk, Korea}
\newcommand{\KSU}{Kansas State University, Manhattan, KS, USA}
\newcommand{\Kyiv}{Taras Shevchenko National University of Kyiv, 01601 Kyiv, Ukraine}
\newcommand{\NRCKI}{National Research Center Kurchatov Institute, Moscow, Russian Federation}
\newcommand{\JSU}{Jackson State University, Jackson, MS, USA}
\newcommand{\jnu}{Jawaharlal Nehru University, New Delhi 110067,  India}
\newcommand{\JU}{University of Jammu, J$\&$K, India}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YW, United Kingdom}
\newcommand{\LBNL}{Lawrence Berkeley National Laboratory, Berkeley, CA USA}
\newcommand{\LLNL}{Lawrence Livermore National Laboratory, Livermore, CA USA}
\newcommand{\Liverpool}{University of Liverpool, Liverpool L69 7ZE, United Kingdom}
\newcommand{\LANL}{Los Alamos National Laboratory, Los Alamos, NM, USA}
\newcommand{\LIP}{Laboratório de Instrumentação e Física Experimental de Partículas, Lisboa and Coimbra, Portugal}
\newcommand{\LSU}{Louisiana State University, Baton Rouge, LA, USA}
\newcommand{\Lucknow}{University of Lucknow, Lucknow, Uttar Pradesh, India}
\newcommand{\MIT}{Massachusetts Institute of Technology, Cambridge, MA, USA}
\newcommand{\MPA}{Max Planck Institute for Astrophysics, Garching, Germany}
\newcommand{\UMN}{University of Minnesota, Minneapolis, MN, USA}
\newcommand{\MSU}{Michigan State University, East Lansing, MI, USA}
\newcommand{\Duluth}{University of Minnesota Duluth, Duluth, MN, USA}
\newcommand{\UMiss}{University of Mississippi, University, MS, USA}
\newcommand{\UCNCl}{Universidad Católica del Norte, Antofagasta, Chile}
\newcommand{\UND}{University of North Dakota, Grand Forks, ND, USA}
\newcommand{\Manchester}{University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\ND}{University of Notre Dame, Notre Dame, IN USA}
\newcommand{\UNSPMF}{University of Novi Sad, Faculty of Sciences, Novi Sad, Serbia}
\newcommand{\OakRidge}{Oak Ridge National Laboratory, Oak Ridge, TN, USA}
\newcommand{\OSU}{Ohio State University, Columbus, OH, USA}
\newcommand{\OregonState}{Oregon State University, Corvallis, OR, USA}
\newcommand{\Oxford}{University of Oxford, Oxford, UK}
\newcommand{\PNNL}{Pacific Northwest National Laboratory, Richland, WA, USA}
\newcommand{\UTF}{Universidade Tecnológica Federal do Paraná, Curitiba, PR, Brazil}
\newcommand{\UniPR}{University of Parma, Department of Engineering and Architecture, Parma, Italy}
\newcommand{\Pennsylvania}{Pennsylvania State University, University Park, PA, USA}
\newcommand{\Penn}{University of Pennsylvania, Phildelphia, PA, USA}
\newcommand{\Pisa}{University and INFN Sezione di Pisa, Pisa, Italy}
\newcommand{\Princeton}{Princeton University, Princeton, NJ, USA}
\newcommand{\PAU}{Punjab Agricultural University, Ludhiana, India}
\newcommand{\QMUL}{Queen Mary University of London, London E1 4NS, United Kingdom}
\newcommand{\Rochester}{University of Rochester, Rochester, NY, USA}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, USA}
\newcommand{\SJSU}{San Jos\'{e} State University, San Jos\'{e}, CA, USA}
\newcommand{\Sheffield}{University of Sheffield, Department of Physics and Astronomy, Sheffield S3 7RH, United Kingdom}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Stanford University, Menlo Park, CA, USA}
\newcommand{\SDSMT}{South Dakota School of Mines and Technology, Rapid City, SD, USA}
\newcommand{\SMU}{Southern Methodist University, Dallas, TX, USA}
\newcommand{\SU}{Stockholm University, Stockholm, Sweden}
\newcommand{\SBU}{Stony Brook University, Stony Brook, NY, USA}
\newcommand{\UoS}{University of Sussex, Falmer, East Sussex, UK}
\newcommand{\SYR}{Syracuse University, Syracuse, NY, USA}
\newcommand{\TAU}{Tel-Aviv University, Tel-Aviv, Israel}
\newcommand{\TAMU}{Department of Physics and Astronomy, Texas A\& M University, College Station, TX, USA}

\newcommand{\UGTO}{Universidad de Guanajuato, Leon GTO, MX}
\newcommand{\UTA}{University of Texas, Arlington, TX, USA}
\newcommand{\UTC}{University of Toronto, Toronto, Canada}
\newcommand{\TUNL}{Triangle Universities Nuclear Laboratory, Durham, NC, USA}
\newcommand{\UCL}{University College London, London WC1E 6BT, United Kingdom}
\newcommand{\UNICAMP}{Universidade Estadual de Campinas (UNICAMP), Campinas, SP, Brazil}
\newcommand{\UNIFAL}{Universidade Federal de Alfenas (Unifal-MG), Po\c{c}os de Caldas, MG, Brazil}
\newcommand{\UFSCAR}{Universidade Federal de São Carlos (UFSCar), Araras, SP, Brazil}
\newcommand{\UNIFESP}{Universidade Federal de S\~ao Paulo (UNIFESP), Diadema, SP, Brazil}
\newcommand{\UFABC}{Universidade Federal do ABC (UFABC), Santo André, SP, Brazil}
% Was already defined above. Which version do we prefer?
%\newcommand{\UNIFAL}{Federal University of Alfenas (UNIFAL) - Minas Gerais, Alfenas, MG, Brazil}
\newcommand{\UGA}{University Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 38000 Grenoble, France}
\newcommand{\Warwick}{University of Warwick, Coventry, UK}
\newcommand{\Wellesley}{Wellesley College, Physics Department, Wellesley, MA, USA}
\newcommand{\UW}{University of Wisconsin, Madison, WI USA}
\newcommand{\VT}{Center for Neutrino Physics, Virginia Tech, Blacksburg, Virginia, USA}
\newcommand{\YALE}{Yale University, New Haven, CT, USA}
\newcommand{\YorkU}{York University, Toronto, ON, Canada}

\newcommand{\ucb}{Physics Department, University of California at Berkeley, Berkeley, CA 94720-7300
}
\newcommand{\lbnl}{
Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720-8153, USA
}
\newcommand{\jul}{Institut f{\"u}r Kernphysik, Forschungszentrum J{\"u}lich, 52425 J{\"u}lich, Germany
}\newcommand{\penn}{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104-6396
}\newcommand{\fcul}{Universidade de Lisboa, Faculdade de Ci{\^e}ncias (FCUL), Departamento de F{\'i}sica, Campo Grande, Edifício C8, 1749-016 Lisboa, Portugal
}\newcommand{\lip}{Laborat{\'o}rio de Instrumenta{}{\c c}{\~a}o e F{\'i}sica Experimental de Part{\'i}culas (LIP), Av. Prof. Gama Pinto, 2, 1649-003, Lisboa, Portugal
}\newcommand{\chic}{
The Enrico Fermi Institute and Department of Physics, The University of Chicago, Chicago, IL 60637, USA
}\newcommand{\bnl}{
Brookhaven National Laboratory, Upton, New York 11973, USA
}\newcommand{\uh}{
University of Hawai‘i at Manoa, Honolulu, Hawai‘i 96822, USA
}\newcommand{\iowa}{
Department of Physics and Astronomy, Iowa State University, Ames, IA 50011, USA
}\newcommand{\jyv}{
Department of Physics, University of Jyv{\"a}skyl{\"a}, Finland
}\newcommand{\ucd}{
University of California, Davis, 1 Shields Avenue, Davis, CA 95616, USA
}\newcommand{\bu}{
Boston University, Department of Physics, Boston, MA 02215, USA
}\newcommand{\mainz}{
Institute of Physics and Excellence Cluster PRISMA, Johannes Gutenberg-Universit{\"a}t Mainz, 55099 Mainz, Germany
}\newcommand{\ham}{
Institut f{\"u}r Experimentalphysik, Universit{\"a}t Hamburg, 22761 Hamburg, Germany
}\newcommand{\alb}{
University of Alberta, Department of Physics, 4-181 CCIS, Edmonton, AB T6G 2E1, Canada
}\newcommand{\pnnl}{
Pacific Northwest National Laboratory, Richland, WA 99352, USA
}\newcommand{\laur}{
Laurentian University, Department of Physics, 935 Ramsey Lake Road, Sudbury, ON P3E 2C6, Canada
}\newcommand{\lsu}{
Department of Physics and Astronomy, Louisiana State University, Baton Rouge, LA 70803
}\newcommand{\tub}{
Kepler Center for Astro and Particle Physics, Universit{\"a}t T{\"u}bingen, 72076 T{\"u}bingen, Germany
}\newcommand{\sheff}{
University of Sheffield, Physics \& Astronomy, Western Bank, Sheffield S10 2TN, UK
}\newcommand{\qu}{
Queen's University, Department of Physics, Engineering Physics \& Astronomy, Kingston, ON K7L 3N6, Canada
}\newcommand{\snolab}{
SNOLAB, Creighton Mine 9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada
}\newcommand{\rut}{
Department of Physics and Astronomy, Rutgers, The State University of New Jersey, 136 Frelinghuysen Road, Piscataway, NJ 08854-8019 USA
}\newcommand{\temp}{
Department of Physics, Temple University, Philadelphia, PA, USA
}\newcommand{\ucla}{
University of California Los Angeles, Department of Physics \& Astronomy, 475 Portola Plaza, Los Angeles, CA 90095-1547, USA
}
\newcommand{\tri}{
SISSA/INFN, Via Bonomea 265, I-34136 Trieste, Italy
}\newcommand{\kav}{
Kavli IPMU (WPI), University of Tokyo, 5-1-5 Kashiwanoha, 277-8583 Kashiwa, Japan
}\newcommand{\kor}{
Center for Underground Physics, Institute for Basic Science, Daejeon 34126, Korea
}\newcommand{\uci}{
University of California, Irvine, Department of Physics, CA 92697, Irvine, USA
}\newcommand{\aach}{
Physikzentrum RWTH Aachen, Otto-Blumenthal-Stra{\ss}e, 52074 Aachen, Germany
}\newcommand{\sbu}{
State University of New York at Stony Brook, Department of Physics and Astronomy, Stony Brook, New York, USA
}\newcommand{\tsing}{
Department of Engineering Physics, Tsinghua University, Beijing 100084, China
}\newcommand{\corn}{
Cornell University, Ithaca, NY, USA
}\newcommand{\boul}{
University of Colorado at Boulder, Department of Physics, Boulder, Colorado, USA
}\newcommand{\dres}{
Institut f{\"u}r Kern und Teilchenphysik, TU Dresden, Zellescher Weg 19, 01069, Dresden, Germany
}
%\newcommand{\mun}{Physik-Department and Excellence Cluster Universe, Technische Universit{\"a}t M{\"u}nchen, 85748 Garching, Germany}
\newcommand{\mun}{Physics Department, Technische Universit{\"a}t M{\"u}nchen, 85748 Garching, Germany
}
\newcommand{\mitnew}{
Massachusetts Institute of Technology, Department of Physics and Laboratory for Nuclear Science, 77 Massachusetts Ave Cambridge, MA 02139, USA
}
\newcommand{\kings}{King’s College London, Department of Physics, Strand Building, Strand, London WC2R 2LS, UK}
\newcommand{\llnl}{
Lawrence Livermore National Laboratory, Livermore, CA 94550, USA
}
\newcommand{\fnal}{
Fermi National Accelerator Laboratory, Batavia, IL 60510, USA
}
\newcommand{\erc}{Department of Physics, Erciyes University, 38030, Kayseri, Turkey
}
\newcommand{\iow}{Department of Physics and Astronomy, The University of Iowa, Iowa City, Iowa, USA}


%\newcommand{\psu}{Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA}
%\newcommand{\psup}{Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA}
\newcommand{\psu}{Pennsylvania State University, University Park, PA 16802, USA}

\newcommand{\heid}{Ruprecht-Karls-Universitat Heidelberg, Im
Neuenheimer Feld 227, Heidelberg, Germany}

\newcommand{\bart}{Bartoszek Engineering, Aurora, IL 60506, USA}

\newcommand{\ucbne}{Nuclear Engineering Department, University of California at Berkeley, Berkeley, CA 94720-7300
}
% \newcommand{\Other}{Other Affiliation.}

% 2nd Block of Commands
% Enter an affiliation directive for each newcommand you entered above. Please make sure it preserves the alphabetical order above.
%\affiliation{\UA}
%\affiliation{\ANL}
%\affiliation{\APC}
%\affiliation{\Atlantico}
%\affiliation{\UBERN}
%\affiliation{\BEU}
%\affiliation{\BU}
%\affiliation{\BNL}
%\affiliation{\BHU}
%\affiliation{\UB}
%\affiliation{\oB}
%\affiliation{\UoBham}
%\affiliation{\Caltech}
\affiliation{\UCB}
\affiliation{\UCD}
\affiliation{\UNC}
\affiliation{\UCI}
\affiliation{\JGU}
%\affiliation{\UCSB}
%\affiliation{\Cambridge}
%\affiliation{\Catania}
%\affiliation{\CERN}
%\affiliation{\CIEMAT}
%\affiliation{\Cincinnati}
%\affiliation{\CUSB}
%\affiliation{\Cinvestav}
%\affiliation{\Columbia}
%\affiliation{\CSU}
%\affiliation{\Drexel}
%\affiliation{\Duke}
%\affiliation{\EDI}
%\affiliation{\EIA}
%\affiliation{\FCUL}
%\affiliation{\FNAL}
%\affiliation{\UF}
%\affiliation{\UGR}
%\affiliation{\Harvard}
%\affiliation{\Hawaii}
%\affiliation{\Houston}
%\affiliation{\ISU}
%\affiliation{\IU}
%\affiliation{\IFIC}
%\affiliation{\IIT}
%\affiliation{\IITH}
%\affiliation{\CzechAcademyofSciences}
%\affiliation{\INFNMiB}
%\affiliation{\INFNNA}
%\affiliation{\INFNGE}
%\affiliation{\Insubria}
%\affiliation{\UOH}
\affiliation{\Iowa}
%\affiliation{\ISP}
%\affiliation{\IowaU}
%\affiliation{\Irfu}
%\affiliation{\Iwate}
%\affiliation{\jnu}
%\affiliation{\JBNU}
%\affiliation{\JSU}
%\affiliation{\JU}
%\affiliation{\KSU}
%\affiliation{\Kyiv}
%\affiliation{\NRCKI}
%\affiliation{\Lancaster}
%\affiliation{\LBNL}
\affiliation{\LLNL}
%\affiliation{\Liverpool}
%\affiliation{\LANL}
%\affiliation{\LIP}
%\affiliation{\LSU}
%\affiliation{\Lucknow}
%\affiliation{\Manchester}
%\affiliation{\MIT}
%\affiliation{\MPA}
%\affiliation{\UMN}
%\affiliation{\Duluth}
%\affiliation{\UMiss}
%\affiliation{\UCNCl}
%\affiliation{\UND}
%\affiliation{\ND}
%\affiliation{\UNSPMF}
%\affiliation{\OakRidge}
%\affiliation{\OSU}
%\affiliation{\OregonState}
\affiliation{\Oxford}
%\affiliation{\PNNL}
%\affiliation{\UniPR}
\affiliation{\Pennsylvania}
\affiliation{\Penn}
%\affiliation{\UTF}
%\affiliation{\PAU}
%\affiliation{\Pisa}
%\affiliation{\Princeton}
%\affiliation{\QMUL}
%\affiliation{\Rochester}
%\affiliation{\Rutgers}
%\affiliation{\SJSU}
%\affiliation{\Sheffield}
%\affiliation{\SLAC}
%\affiliation{\SDSMT}
%\affiliation{\SMU}
%\affiliation{\SU}
%\affiliation{\SBU}
%\affiliation{\UoS}
%\affiliation{\SYR}
%\affiliation{\TAU}
%\affiliation{\TAMU}
%\affiliation{\UGTO}
%\affiliation{\UTA}
%\affiliation{\UTC}
\affiliation{\TUNL}
%\affiliation{\UCL}
%\affiliation{\UNICAMP}
%\affiliation{\UNIFAL}
%\affiliation{\UFSCAR}
%\affiliation{\UNIFESP}
%\affiliation{\UFABC}
%\affiliation{\UGA}
%\affiliation{\UNIFAL}
%\affiliation{\Warwick}
%\affiliation{\Wellesley}
%\affiliation{\UW}
%\affiliation{\VT}
%\affiliation{\YALE}
%\affiliation{\YorkU}


% \affiliation{\Other}

%3rd Block of Commands, divided by "Editors", "Contributors", and "All Other Authors/Endorsers"

% Lead Editors go here in alphabetical order with affiliation indexed by %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT ADD YOUR NAME TO THIS SECTION unless you were an editor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \author{\\A.~N.~Author}
% \affiliation{\Other}

\author{Joshua~Klein}
\altaffiliation{\Editor}
\affiliation{\Penn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT ADD YOUR NAME ABOVE THIS LINE unless you were an editor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT ADD NAME TO THIS NEXT SECTION unless you were a primary contributor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Contributing authors go here in new alphabetical order with affiliation indexed by \dagger

%\author{A.~Person}
%\altaffiliation{\Contributor}
%\affiliation{\IIT}

\author{Tomi Akindele}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Adam Bernstein}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Steven Biller}
\altaffiliation{\Contributor}
\affiliation{\Oxford}

\author{Nathaniel Bowden}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Jason Brodsky}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{D.F.~Cowen}
\altaffiliation{\Contributor}
\affiliation{\Pennsylvania}

\author{Michael Ford}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Julieta Gruszko}
\altaffiliation{\Contributor}
\affiliation{\UNC}
\affiliation{\TUNL}

\author{Logan Lebanowski}
\altaffiliation{\Contributor}
\affiliation{\Penn}

\author{Aobo Li}
\altaffiliation{\Contributor}
\affiliation{\UNC}
\affiliation{\TUNL}

\author{Viacheslav A. Li}
\altaffiliation{\Contributor}
\affiliation{\LLNL}

\author{Wei Mu}
\altaffiliation{\Contributor}
\affiliation{\FNAL}

\author{J. Pedro Ochoa-Ricoux}
\altaffiliation{\Contributor}
\affiliation{\UCI}

\author{Gabriel~D.~Orebi~Gann}
\altaffiliation{\Contributor}
\affiliation{\UCB}
\affiliation{\LBNL}

\author{Mayly Sanchez}
\altaffiliation{\Contributor}
\affiliation{\Iowa}

\author{Robert Svoboda}
\altaffiliation{\Contributor}
\affiliation{\UCD}

\author{Matthew Wetstein}
\altaffiliation{\Contributor}
\affiliation{\Iowa}

\author{Michael Wurm}
\altaffiliation{\Contributor}
\affiliation{\JGU}

\author{Minfang Yeh}
\altaffiliation{\Contributor}
\affiliation{\BNL}

\collaboration{Editors and Contributors}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DO NOT ADD NAME ABOVE HERE unless you were an primary contributor!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% All Other Authors go here in new alphabetical order with affiliation,
%broken down by Collaboration if relevant

%If you are signing as an individual from Theia, please put your name below this line and
%above the \collaboration{} line below with Theia in it 

%\author{B.~Person}
%\affiliation{\IIT}
\author{M.~Askins}\affiliation{\ucb}\affiliation{\lbnl}
\author{Z.~Bagdasarian}\affiliation{\ucb}\affiliation{\lbnl}
\author{N.~Barros}\affiliation{\penn}
\affiliation{\fcul}
\affiliation{ \lip}
\author{E.W.~Beier}\affiliation{\penn}
\author{A.~Bernstein}\affiliation{\llnl}
\author{M.~B\"ohles}\affiliation{\mainz}
\author{E.~Blucher}\affiliation{\chic}
\author{R.~Bonventre}\affiliation{\lbnl}
\author{E.~Bourret}\affiliation{\lbnl}
\author{E.~J.~Callaghan}\affiliation{\ucb}\affiliation{\lbnl}
\author{J.~Caravaca}\affiliation{\ucb}\affiliation{\lbnl}
\author{M.~Diwan}\affiliation{\bnl}
\author{S.T.~Dye}\affiliation{\uh}
\author{J.~Eisch}\affiliation{\fnal}
\author{A.~Elagin}\affiliation{\chic}
\author{T.~Enqvist}\affiliation{\jyv}
\author{U.~Fahrendholz}\affiliation{\mun}
\author{V.~Fischer}\affiliation{\ucd}
\author{K.~Frankiewicz}\affiliation{\bu}
\author{C.~Grant}\affiliation{\bu}
\author{D.~Guffanti}\affiliation{\mainz}
\author{C.~Hagner}\affiliation{\ham}
\author{A.~Hallin}\affiliation{\alb}
\author{C.~M.~Jackson}\affiliation{\pnnl}
\author{R.~Jiang}\affiliation{\chic}
\author{T.~Kaptanoglu}\affiliation{\ucb}\affiliation{\lbnl}
\author{J.R.~Klein}\affiliation{\penn}
\author{Yu.~G.~Kolomensky}\affiliation{\ucb}\affiliation{\lbnl}
\author{C.~Kraus}\affiliation{\laur}
\author{F.~Krennrich}\affiliation{\iowa}
\author{T.~Kutter}\affiliation{\lsu}
\author{T.~Lachenmaier}\affiliation{\tub}
\author{B.~Land}\affiliation{\ucb}\affiliation{\lbnl}\affiliation{\penn}
\author{K.~Lande}\affiliation{\penn}
\author{L.~Lebanowski}\affiliation{\penn}
\author{J.G.~Learned}\affiliation{\uh}
\author{V.A.~Li}\affiliation{\llnl}
\author{V.~Lozza}\affiliation{\fcul}
\affiliation{ \lip}
\author{L.~Ludhova}\affiliation{\jul}\affiliation{\aach}
\author{M.~Malek}\affiliation{\sheff}
\author{S.~Manecki}\affiliation{\laur}\affiliation{\qu}\affiliation{\snolab}
\author{J.~Maneira}\affiliation{\fcul}
\affiliation{ \lip}
\author{J.~Maricic}\affiliation{\uh}
\author{J.~Martyn}\affiliation{\mainz}
\author{A.~Mastbaum}\affiliation{\rut}
\author{C.~Mauger}\affiliation{\penn}
\author{M.~Mayer}\affiliation{\mun}
\author{J.~Migenda}\affiliation{\kings}
\author{F.~Moretti}\affiliation{\lbnl}
\author{J.~Napolitano}\affiliation{\temp}
\author{B.~Naranjo}\affiliation{\ucla}
\author{S.~Naugle}\affiliation{\penn}
\author{M.~Nieslony}\affiliation{\mainz}
\author{L.~Oberauer}\affiliation{\mun}
\author{G.~D.~Orebi~Gann}\affiliation{\ucb}\affiliation{\lbnl}
\author{J.~Ouellet}\affiliation{\mitnew}
\author{T.~Pershing}\affiliation{\ucd}
\author{S.T.~Petcov}\affiliation{\tri,\kav}
\author{L.~Pickard}\affiliation{\ucd}
\author{R.~Rosero}\affiliation{\bnl}
\author{M.~C.~Sanchez}\affiliation{\iowa}
\author{J.~Sawatzki}\affiliation{\mun}
\author{S.~Schoppmann}\affiliation{\ucb}\affiliation{\lbnl}
\author{S.H.~Seo}\affiliation{\kor}
\author{M.~Smiley}\affiliation{\ucb}\affiliation{\lbnl}
\author{M.~Smy}\affiliation{\uci}
\author{A.~Stahl}\affiliation{\aach}
\author{H.~Steiger}\affiliation{\mainz}\affiliation{\mun}
\author{M.~R.~Stock}\affiliation{\mun}
\author{H.~Sunej}\affiliation{\bnl}
\author{R.~Svoboda}\affiliation{\ucd}
\author{E.~Tiras}\affiliation{\erc}\affiliation{\iow}
\author{W.~H.~Trzaska}\affiliation{\jyv}
\author{M.~Tzanov}\affiliation{\lsu}
\author{M.~Vagins}\affiliation{\uci}
\author{C.~Vilela}\affiliation{\sbu}
\author{Z.~Wang}\affiliation{\tsing}
\author{J.~Wang}\affiliation{\ucd}
\author{M.~Wetstein}\affiliation{\iowa}
\author{M.J.~Wilking}\affiliation{\sbu}
\author{L.~Winslow}\affiliation{\mitnew}
\author{P.~Wittich}\affiliation{\corn}
\author{B.~Wonsak}\affiliation{\ham}
\author{E.~Worcester}\affiliation{\bnl}\affiliation{\sbu}
\author{M.~Wurm}\affiliation{\mainz}
\author{G.~Yang}\affiliation{\sbu}
\author{M.~Yeh}\affiliation{\bnl}
\author{E.D.~Zimmerman}\affiliation{\boul}
\author{S.~Zsoldos}\affiliation{\ucb}\affiliation{\lbnl}
\author{K.~Zuber}\affiliation{\dres}

\collaboration{Co-Signers from \theia}
\noaffiliation

%If you are signing as an individual from WATCHMAN, please put your name below this line and
%above the \collaboration{} line below with WATCHMAN in it 

\collaboration{Co-Signers from WATCMAN}

%If you are signing as an individual from Eos, please put your name below this line and
%above the \collaboration{} line below with Eos in it 

\author{T.~Anderson}\affiliation{\psu}
\author{E.~Anderssen}\affiliation{\lbnl}
\author{M.~Askins}\affiliation{\lbnl}\affiliation{\ucb}
\author{A.~J.~Bacon}\affiliation{\penn}
\author{Z.~Bagdasarian}\affiliation{\lbnl}\affiliation{\ucb}
\author{A.~Baldoni}\affiliation{\psu}
\author{N.~Barros}\affiliation{\fcul}\affiliation{ \lip}
\author{L.~Bartoszek}\affiliation{\bart}
\author{A.~Bat}\affiliation{\erc}
\author{M.~Bergevin}\affiliation{\llnl}
\author{A.~Bernstein}\affiliation{\llnl}
\author{E.~Blucher}\affiliation{\chic}
\author{J.~Boissevain}\affiliation{\bart}
\author{R.~Bonventre}\affiliation{\lbnl}
\author{D.~Brown}\affiliation{\lbnl}
\author{E.~J.~Callaghan}\affiliation{\lbnl}\affiliation{\ucb}
\author{D.~F.~Cowen}\affiliation{\psu}
\author{S.~Dazeley}\affiliation{\llnl}
\author{M.~Diwan}\affiliation{\bnl}
\author{M.~Dunford}\affiliation{\heid}
\author{K.~Frankiewicz}\affiliation{\bu}
%\author{B.~Goldblum}\affiliation{\lbnl}\affiliation{\ucbne}
\author{C.~Grant}\affiliation{\bu}
\author{T.~Kaptanoglu}\affiliation{\lbnl}\affiliation{\ucb}
\author{J.R.~Klein}\affiliation{\penn}
\author{C.~Kraus}\affiliation{\laur}
\author{T.~Kroupa}\affiliation{\penn}
\author{B.~Land}\affiliation{\lbnl}\affiliation{\ucb}\affiliation{\penn}
\author{L.~Lebanowski}\affiliation{\penn}
\author{V.~Lozza}\affiliation{\fcul}\affiliation{ \lip}
\author{A.~Marino}\affiliation{\boul}
\author{A.~Mastbaum}\affiliation{\rut}
\author{C.~Mauger}\affiliation{\penn}
\author{S.~Naugle}\affiliation{\penn}
\author{M.~Newcomer}\affiliation{\penn}
\author{A.~Nikolica}\affiliation{\penn}
\author{G.~D.~Orebi~Gann}\affiliation{\lbnl}\affiliation{\ucb}
\author{L.~Pickard}\affiliation{\ucd}
\author{J.~Saba}\affiliation{\lbnl}
\author{S.~Schoppmann}\affiliation{\lbnl}\affiliation{\ucb}
\author{J.~Sensenig}\affiliation{\penn}
%\author{Z.~Siegel}\affiliation{\chic}
\author{M.~Smiley}\affiliation{\lbnl}\affiliation{\ucb}
\author{H.~Steiger}\affiliation{\mainz}\affiliation{\mun}
\author{R.~Svoboda}\affiliation{\ucd}
\author{E.~Tiras}\affiliation{\erc}\affiliation{\iow}
\author{W.~H.~Trzaska}\affiliation{\jyv}
\author{R.~van~Berg}\affiliation{\penn}\affiliation{\bart}
\author{G.~Wendel}\affiliation{\psu}
\author{M.~Wetstein}\affiliation{\iowa}
\author{M.~Wurm}\affiliation{\mainz}
\author{G.~Yang}\affiliation{\lbnl}\affiliation{\ucb}
\author{M.~Yeh}\affiliation{\bnl}
\author{E.D.~Zimmerman}\affiliation{\boul}
\collaboration{Co-Signers from Eos}

%If you are signing as an individual from SNO+, please put your name below this line and
%above the \collaboration{} line below with SNO+ in it 

\collaboration{Co-Signers from SNO+}

%If you are signing as an individual from Eos, please put your name below this line and
%above the \collaboration{} line below with WATCHMAN in it 
